Leveraging Foundation Models for Zero-Shot IoT Sensing

Deep learning models are increasingly deployed on edge Internet of Things (IoT) devices. However, these models typically operate under supervised conditions and fail to recognize unseen classes different from training. To address this, zero-shot learning (ZSL) aims to classify data of unseen classes with the help of semantic information. Foundation models (FMs) trained on web-scale data have shown impressive ZSL capability in natural language processing and visual understanding. However, leveraging FMs' generalized knowledge for zero-shot IoT sensing using signals such as mmWave, IMU, and Wi-Fi has not been fully investigated. In this work, we align the IoT data embeddings with the semantic embeddings generated by an FM's text encoder for zero-shot IoT sensing. To utilize the physics principles governing the generation of IoT sensor signals to derive more effective prompts for semantic embedding extraction, we propose to use cross-attention to combine a learnable soft prompt that is optimized automatically on training data and an auxiliary hard prompt that encodes domain knowledge of the IoT sensing task. To address the problem of IoT embeddings biasing to seen classes due to the lack of unseen class data during training, we propose using data augmentation to synthesize unseen class IoT data for fine-tuning the IoT feature extractor and embedding projector. We evaluate our approach on multiple IoT sensing tasks. Results show that our approach achieves superior open-set detection and generalized zero-shot learning performance compared with various baselines. Our code is available at https://github.com/schrodingho/FM\_ZSL\_IoT.

==> motivation.tex <==
{\red \textbf{To be deleted}}
Challeng 1: text embeddings generated by frozen FM's text encoder gather together, which affects IoT embedding's separability/FM's text encoder cannot efficiently generalize to fine-grained downstream tasks -> external expert knowledge and prompt tuning/learnable prompt

{\red Fig.1 T-SNEs of the text and IoT embeddings for seen classes with and without prompt tuning}

Challenge 2: unseen IoT embeddings biased to seen IoT embeddings due to small volume of training data -> synthesized unseen data using generative model

{\red Fig. 2 T-SNEs of text and IoT embeddings for seen and unseen classes with and without GAN-based data augmentation.}

\begin{figure}
    \centering
    \includegraphics[width=.8\columnwidth]{figs/two_t-SNE.png}
    \caption{place holder}
    
    \label{fig:t-SNE}
\end{figure}

\begin{table}[]
\begin{tabular}{ll}
 Specialist DNN & $f(\cdot)$ \\
 Foundation model & $\Phi(\cdot)$ \\
 Set of seen classes & $\mathcal{S} = \{c_i^s\}_{i = 1}^{N_s}$ \\
 Seen train set & $D^s = \{(\vec{x}^s_i, y^s_i)\}^{N_{train}}_{i = 1} \in \mathcal{X} \times \mathcal{S}$ \\
 Seen IoT data $i$ & $\vec{x}^s_i \in \mathbb{R}^d$ \\
 Seen IoT data $i$ label & $y^s_i$\\
 Set of unseen classes & $\mathcal{U} = \{c_i^u\}_{i = 1}^{N_u}$ \\
 Test set & $D^s = \{\vec{x}^\text{test}_i\}^{N_{test}}_{i = 1} \in \mathcal{X}$ \\
 CLIP's text encoder & $\Phi_{\text {text}}(\cdot)$ \\
 Learnable soft prompt of class $c$ & $\vec{p}^l(c) = \oplus (\vec{l}_1, ..., {\text {CLIPtokenizer}}[c] , ..., \vec{l}_M)$ \\
 $\vec{l}_i$ & $i$th learnable token\\
 Learnable text embedding of class $c$ & $\vec{t}^l(c) = \Phi_{\text {text}}(\vec{p}^l(c))$\\
 Auxiliary hard prompt of class $c$ & $\vec{p}^a(c)$ \\
 Auxiliary text embedding of class $c$ & $\vec{t}^a(c) = \Phi_{\text {text}}(\vec{p}^a(c))$\\
 Query input & $\vec{Q} = \rho_{\vec{Q}}(\vec{t}^a)$ \\
 Key input & $ \vec{K} = \rho_{\vec{K}}(\vec{t}^l)$ \\
 Value input & $\vec{V} = \rho_{\vec{V}}(\vec{t}^l)$ \\
 fully-connected layers in cross-attention\\ module & $\rho_k(\cdot), (k \in \{\vec{Q}, \vec{K}, \vec{V}\}$)  \\
 Attention weights & $\vec{A} = \text {softmax}(\frac{\vec{Q} \vec{K}^T}{\sqrt{d_k}})$, \\
 Dimension of $\vec{K}$ & $d_\vec{K}$ \\
 Class prototype/text embedding & $\vec{t} = \vec{A}\vec{V}$ \\
 Semantic space & $\mathcal{T} = \{\vec{t}(c) \mid c \in \mathcal{S} \cup \mathcal{U}\}$ \\
 IoT feature extractor& $\mu(\cdot)$ \\
 IoT feature & $\vec{h}_i = \mu(\vec{x}_i)$\\
 IoT embedding projector & $g(\cdot)$ \\
 IoT embedding & $\vec{e}_i = g(\vec{h}_i)$ \\
 A batch of train data sampled from $D^s$ & $\{(\vec{x}^s_i, y^s_i)\}^{N_B}_{i = 1}$ \\
 Index of the data in a train batch & $i \in I \equiv \{1 \cdots N_B\}$\\
 \# of distinct classes in a train batch & $N_T$ \\
 Index of distinct classes in a train batch & $j \in J \equiv \{1 \cdots N_T\}$ \\
 Supervised contrastive loss & $\mathcal{L}$\\
 Generator for data aug & $G(\cdot)$ \\
 Random Gaussian noise vector & $\vec{z}$ \\
 Synthesized IoT data & $\tilde{\vec{x}} \in \mathcal{X}$ \\
 Discriminator for data aug & $D(\cdot)$ \\
 Penalty coefficient in data aug & $\lambda$\\
 linear softmax classifier in data aug & $\theta$\\
 GAN loss in data aug & $\mathcal{L}_\text{WGAN}$\\
 Cls loss in data aug & $\mathcal{L}_\text{CLS}$\\
 data aug loss & $\mathcal{L}_\text{DA}$\\
 synthesized unseen train set & $D^{aug} = \{(\tilde{\vec{x}}^u_i,y^u_i)\}^{N_{aug}}_{i = 1} \in \mathcal{X} \times \mathcal{U}$\\
 Class clusters of seen IoT embeddings & $\{E^s_i\}^{N_s}_{i=1}$ \\
 IoT embeddings in each seen class cluster & $\{\vec{e}_{i,j}\}_{j=1}^{N_i}$\\
 Input data sample & $\vec{x}^\text{test}$ \\
 Input data IoT embedding & $\vec{e}^{\text{test}}$ \\
 Euclidean distances btw $\vec{e}^{\text{test}}$ and $\{\vec{e}_{i,j}\}_{j=1}^{N_i}$ & $d_{i,j} = \Vert \vec{e}^{\text{test}} - \vec{e}_{i,j} \Vert_2, \vec{e}_{i,j} \in E^s_i$\\
 $k$-th smallest distance for each cluster & $d_i^{(k)}$ \\
 class-specific distance threshold & $\lambda_i$ \\
 detected ``unseen'' test sample & $\vec{x}^{\text{det}}$ \\
 detected ``unseen'' test IoT embedding & $\vec{e}^{\text{det}}$ \\
 predicted label for $\vec{x}^{\text{det}}$ & $\hat{y}^{\text{det}}$\\
\end{tabular}
\caption{\red to be deleted. for ref only}
\end{table}











